TF2AIF: Facilitating development and deployment of accelerated AI models on the cloud-edge continuum

The B5G/6G evolution relies on connect-compute technologies and highly heterogeneous clusters with HW accelerators, which require specialized coding to be efficiently utilized. The current paper proposes a custom tool for generating multiple SW versions of a certain AI function input in high-level language, e.g., Python TensorFlow, while targeting multiple diverse HW+SW platforms. TF2AIF builds upon disparate tool-flows to create a plethora of relative containers and enable the system orchestrator to deploy the requested function on any peculiar node in the cloud-edge continuum, i.e., to leverage the performance/energy benefits of the underlying HW upon any circumstances. TF2AIF fills an identified gap in today's ecosystem and facilitates research on resource management or automated operations, by demanding minimal time or expertise from users.

==> IEEEtran5/sections/tf2aif2.tex <==
\AT{\subsection{Details-v2}}

Figure 2 illustrates the overview of TF2AIF, using the generation of AIFs for a far-edge node platform, i.e., NVIDIA Jetson AGX.
More specifically, the user provides inputs to the converter (\circled{1}). 
The \textit{Converter} produces the required model (\circled{2}).
Finally, the Composer, using the user-provided configuration files (\circled{3}), and some additional boilerplate code (\circled{4}) generates the AI inference service (\circled{5}).

The components, as well as the features of our tool, are thoroughly described in the rest of this subsection.

\textbf{Converter:}
The Converter is a platform-specific component that is responsible for the conversion of the given TensorFlow model to the appropriate format, e.g., ONNX runtime.
Additionally, inference acceleration frameworks facilitate or necessitate model quantization, a process where the model's weights are converted from the standard FP32 format to either FP16 or INT8. 
This transformation optimizes the model for more efficient processing and performance on hardware accelerators.
This process requires a calibration dataset with inputs that are representative of the inputs that will be used on the specific model. 
The Converter provides an interface that unburdens the user from transforming the dataset to the required AI framework format.
The user only needs to provide the dataset in the \texttt{tf.data.Dataset} form.

\textbf{Composer:}
Next, the Composer is the second stage of the model-variant generation.
At this stage, user-provided input, i.e., configuration files, interface implementation, and TF2AIF platform-specific code are combined with the consistent across all platforms and models Base Server Code (Fig. \ref{fig_tf2aif_agx_single_example}).

The platform- and AI-framework-specific components are the converted model from the previous stage (\circled{}), Base Server, and Base Image.
The Base Server provides a class with specific functionality for the target framework-platform combination. 
It includes methods that correspond to server initialization configurations and the model execution, while also supporting request queuing.
% Base Server also supports request queuing 
The standardization of the Base Server decouples the server functionality that depends on the AI-framework-platform intricacies from the functionality that is independent of the combination. 
This makes the design more modular and enhances the extensibility of the framework by simplifying the process of introducing new framework-platform combinations to TF2AIF.

To streamline the process of model-variant generation, we provide a container template (Base Image) that sets the environment of the resulting AIF.
While each AI framework and platform combination needs to adhere to specific environment requirements, our focus is on minimizing these differences.
To achieve this, we select the same libraries and environmental variable configurations, where possible.
This eliminates any noise introduced by variable library versions, etc when experimenting with different model variants.
This feature is critical when TF2AIF is employed for hardware/model performance evaluation.

The other input of the Composer is the user-provided input, as illustrated in the blue-shaded area in Fig. \ref{fig_tf2aif_agx_single_example}.
More specifically, the user can implement an interface related to the pre/post-processing of data, as well as provide configuration files for customization.
TF2AIF aiming to minimize the user intervention as much as possible, 
provides methods that implement functionality that changes per model such as the pre/post-processing functions.
\AT{XXX}
In the evaluated model variants (\S \ref{sec:evaluation}), this interface was completed using only 100 lines of elementary Python scripting. 
This interface is reused across all framework-platform implementations.
One more key design feature of the TF2AIF framework is the volume of customization options it provides.
Users can optionally define their custom specifications.
Those specifications include networking-related information, e.g., IP address, model-related, e.g., the batch size, or framework-related, e.g., precision and parallelization factors.
TF2AIF is highly extensible, allowing users to add external files, libraries, and environmental variables.



\textbf{Additional Components:}
% \begin{itemize}
%     \item metrics server / statistics / logging
%     \item client
%     \item queuing
% \end{itemize}
A key feature of TF2AIF is metrics collection.
The AIF server, except for the endpoint that responds to AI inference requests, includes an additional endpoint that returns metrics.
More specifically, the AIF server during execution monitors the resulting metrics, e.g., latency, and throughput.
Therefore, ad-hoc, through the specified endpoint, clients have access to performance statistics such as average throughput or the 90$^{th}$ percentile of latency.


TF2AIF, along with the AIF server, also generates the implementations of the respective clients, for completeness, AIF server verification, and to further simplify benchmarking, 
The client-server communication is conducted using the REST API.
The client container is created by a separate composer.
Similarly to the aforementioned composer for the server, it requires configuration files and some interface implementation code as input.
The user needs to implement the interface that manages the type of server input and output data. 
Creating this example client is pivotal in both the verification and the quick deployment of the server containers.
client-server communication through the REST API that is. 

\subsection{Benefits outline}


% The composer contains the Base Server Class code, which provides foundational server functionality that is consistent across all platforms and models.
% It implements a Flask server that provides two endpoints for an inference service and a metrics service.
% A client can access the inference service endpoint to request a serving. 
% The Base Server Class implements a worker thread that is responsible of managing requests via a queuing mechanism.
% After each serving, the server calculates some benchmarking metrics, such as latency and throughput and keeps a record of the statistics of all the requests. 
% Then the client can access the metrics service endpoint and request this information. 
% Additionally, the Base Server Class is responsible for all the logging functionality of the server as well as initializing some server configurations.


